Asymptotic Degradation of Linear Regression Estimates With Strategic Data Sources

We consider the problem of linear regression from strategic data sources with a public good component, i.e., when data is provided by strategic agents who seek to minimize an individual provision cost for increasing their data's precision while benefiting from the model's overall precision. In contrast to previous works, our model tackles the case where there is uncertainty on the attributes characterizing the agents' data -- a critical aspect of the problem when the number of agents is large. We provide a characterization of the game's equilibrium, which reveals an interesting connection with optimal design. Subsequently, we focus on the asymptotic behavior of the covariance of the linear regression parameters estimated via generalized least squares as the number of data sources becomes large. We provide upper and lower bounds for this covariance matrix and we show that, when the agents' provision costs are superlinear, the model's covariance converges to zero but at a slower rate relative to virtually all learning problems with exogenous data. On the other hand, if the agents' provision costs are linear, this covariance fails to converge. This shows that even the basic property of consistency of generalized least squares estimators is compromised when the data sources are strategic.

==> related-work.tex <==
% !TEX root = aaai.tex



% , which shows that GLS is no longer optimal when data sources have heterogeneous provision costs. In our work, we use a similar model but we crucially assume that agents do not know the independent variables $x_i$ of others but only their distribution. We then focus on asymptotic decay and consistency of GLS estimates rather than on their optimality. Similar to \cite{Gast20a} (but unlike all other works on strategic data sources), we assume that the precision of the data provided by each agent is known to the analyst performing the linear regression. Indeed, as there is no payment in our model and as agents are motivated to decrease the GLS covariance estimates, there is no a priori reason for the agents to misreport it---we leave a more formal development of this argument to future work. 


%\paragraph{Strategic regression}

%\paragraph{Optimal design}

%In optimal design \cite{pukelsheim2006optimal,atkinson2007optimum,boyd2004convex}, an analyst chooses the $x_i$'s of the set of (non-strategic) data sources, to maximize the quality of the linear model estimated via a scalarization of the covariance matrix. Following this approach, we also use a scalarization of the covariance to measure the model's precision and we borrow scalarization corresponding to classical optimal design criteria (e.g., A-optimality or E-optimality). In contrast, however, we consider strategic data sources and assume that the $x_i$'s are drawn i.i.d. from a given distribution. Interestingly, we will show that in certain cases, the distribution of precision over the set of $x_i$'s that results from the equilibrium of our game-theoretic model does match an optimal design. 


%\paragraph{Federated learning}
 
%An important motivating example of our model is in the context of federated learning (see a survey in \cite{yang2019federated}). In such a context, each agent performs a local estimation and these estimations are combined by an analyst to obtain a model. This paradigm can be used for reason of efficiency (there are many agents, each capable of a local optimization \cite{konevcny2016federated}) or privacy (all agents want to compute a joint representative model without explicitly having to share their personal data \cite{geyer2017differentially}). Our model can be viewed as an instance of both cases. In a distributed recommender  system, agents would be interested to know what affects the good rating of a restaurant but prefer to avoid contributing (for instance because it takes time). In a medical context, a group of hospitals could want to share their data in order to estimate precisely the influence of various patients characteristics on some diseases. Yet, for privacy or cost reasons (gathering data about many patients takes time), each hospital might want to avoid providing very precise estimates. Our work tackles a question unexplored in those federated learning works: how does the public good component of the model learned collaboratively affects the result?





%%% Local Variables:
%%% mode: latex
%%% TeX-master: "nips.tex"
%%% End:

